Prompt Combines Paraphrase: Teaching Pre-trained Models to Understand Rare Biomedical Words

Prompt-based fine-tuning for pre-trained models has proven effective for many natural language processing tasks under few-shot settings in general domain. However, tuning with prompt in biomedical domain has not been investigated thoroughly. Biomedical words are often rare in general domain, but quite ubiquitous in biomedical contexts, which dramatically deteriorates the performance of pre-trained models on downstream biomedical applications even after fine-tuning, especially in low-resource scenarios. We propose a simple yet effective approach to helping models learn rare biomedical words during tuning with prompt. Experimental results show that our method can achieve up to 6% improvement in biomedical natural language inference task without any extra parameters or training steps using few-shot vanilla prompt settings.

==> Table/only-test.tex <==
\begin{table}[H]
%\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}
{%
\begin{tabular}{c|ccccc}
\hline
\hline
\#Samples& 16 & 32 & 64 & 128 & 256 \\
\hline
w/o p-       & 51.3 & 60.6 & 71.0 & 80.6 & 83.1 \\
w/ p-train\&dev   & 49.5 & 56.9 & 62.5 & 76.5 & 82.1 \\
w/ p-test & & & & & \\
w/ p-all & 56.6 & 62.3 & 74.5 & 81.1 & \textbf{83.6} \\
\hline
\hline
\end{tabular}%
}
\caption{Results for few-shot learning through different paraphrasing strategy on MedNLI with the BC-RoBERTa-Large model. w/o p-: without paraphrases for rare biomedical words. w/ paraphrase\dag: with paraphrases for rare biomedical words in test sets. w/ paraphrase: with paraphrases for rare biomedical words in all sets.}
\label{table-only-test}
\end{table}



==> Text/expi_Introduction.tex <==
\section{Introduction}
With the blossom of pre-trained models (PTMs), natural language processing (NLP) have been ushered into a new era \citep{peters2018deep,devlin2019bert,liu2019roberta,qiu2020pre}, along with that in biomedical domain tasks \citep{lee2020biobert,lewis2020pretrained,zhao2021recent}. However, there are two possible obstacles that may hinder the performance of biomedical PTMs, that are limited data and rare biomedical words.

In biomedical domain, it is common that the amount of data is limited due to rare diseases or data sensitivity \citep{vsuster2017short}. For instance, there are around 800 ICD codes in MIMIC-III dataset that have less than 40 hospital admissions while tha dataset contains 53,423 admissions overall \citep{johnson2016mimic}. Meanwhile, biomedical records are usually private data under confidentiality and biomedical data are not easily accessible. Promising results gained by ``Pre-training and Fine-tuning'' model are on the basis of sufficient training steps of additional parameters pertaining to new tasks, such as BERT \citep{devlin2019bert}. Otherwise, PTMs are unlikely to perform well in few-shot settings \citep{moradi2021gpt}. 

With limited tuning data for a new task, it is hard to fine-tune the PTMs and the new task-specific parameters effectively. To solve the above problem, ``Pre-training, Prompt and Predicting'' is proposed to smooth the fine-tuning process in few-shot settings by closing the gap between pre-training stage and the downstream task \citep{liu2021pre}. As demonstrated in Figure \ref{intro_prompt}, tuning with prompt inherits task paradigm from pre-training. Thus, downstream tasks wouldn't be a far cry from the pre-training tasks, which empowers the PTMs to perform better in the case of restricted amount of data.
% transfer to biomedical domain

Furthermore, quantity of specialized rare terms derive from Latin or Greek which are hard to comprehend \citep{keselman2012classification} for both human and PTMs. Besides, an increasing number of biomedical neologisms emerge over time due to biomedical breakthroughs or new diseases, like Covid-19. 

Also, words are generally in long-tail distribution and \citet{schick2020rare,wu2020taking} have discussed that rare words hinder the PTMs to understand sentences correctly. Biomedical rare words, which are semantically more related to biomedical tasks, tend to barrier the biomedical PTMs more. As an example of biomedical NLI task, model goes wrong when faced with a rare words ``\textit{afebrile}''\footnote{There are around 4 billion words in pre-training texts of the BC-RoBERTa-Large and ``afebrile'' appears only about 100,000 times. For comparison, the frequency of ``fever'' is 5 times that of ``afebrile''.} in the premise in Figure \ref{wrong-case} in Appendix \ref{appendix-wrong-case}, whose meaning is ``having no fever''. It's hard for PTMs to predict the label right without knowing ``afebrile''.

Several works alleviate the rare words problem in PTMs via leveraging non-rare words or tokens to approximate rare words \citep{schick2020rare} or injecting knowledge or contexts of certain set of rare words into pre-training procedure to enrich the representation of rare words \citep{yu2021dict,wu2020taking}. Although they have achieved improvement in grasping the meaning of rare words, further pre-training steps are essential for specific rare words. And if a trained model comes across new rare words in another task, extra pre-training will be inevitable. 
 

 


%More recently, PTMs are faced with a profound transformation from ``Pre-training and Fine-tuning'' to ``Pre-training, Prompt and Predicting'', namely prompt-based fine-tuning \citep{liu2021pre}. 

%Fine-tuning solves the downstream tasks with a transfer learning objective engineering from pre-trained targets, which requires sufficient training steps of additional parameters pertaining to new tasks, such as BERT \citep{devlin2019bert}. Although the model above is satisfactory to scenarios with adequate fine-tuning data, PTMs could not perform well in few-shot settings \citep{moradi2021gpt}. 

%Given this, tuning with prompt is proposed to transform downstream tasks from existing fine-tuning to look more like the pre-trained tasks by the help of \textit{prompt} \citep{liu2021pre}   
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{acl-ijcnlp2021-templates/Figure/intro-prompt-neo.pdf}
\caption{Examples for paradigms of (a) MLM (Masked Language Model) Pre-training. (b) Task-specific fine-tuning. (c) Prompt-based fine-tuning, with same task as pre-training process. (d) Paraphrase-enhanced prompt-based fine-tuning. Best viewed in color.}
\label{intro_prompt}
\end{figure*}




In this work, we build upon the recent success of prompt for the PTMs and focus on helping biomedical PTMs understand biomedical terms in the downstream tasks during tuning with prompt by looking them up in the dictionary, which mimics the behavior when human reads as knowledge enhancement. We attach the paraphrases of selected biomedical rare words to the words themselves in the datasets of downstream tasks only during tuning stage via tuning with vanilla prompt without 
extra pre-training. Also, our method is a plug-in module for task datasets and model-agnostic, which can be easily transferred to other domains and models\footnote{We plan to release our code at ...}.

In summary, our main contributions are as follows:
\begin{itemize}
    \item We are the first work to leverage paraphrases of words in the PTM tuning stage to enrich the representation, to the best of our knowledge.
    \item We combine the prompt-based fine-tuning and a portable plug-in module to help understand biomedical  rare words. Afterwards, we evaluate on two biomedical natural language understanding datasets and our approach can improve the performance by up to 5 \% in few-shot settings and 0.6 \% with full-size training dataset.
    \item We discuss how the paraphrases help with the PTMs and provide a novel perspective about task-related rare words.
    
\end{itemize}

==> Text/x.ethics.tex <==
\section*{Ethical Considerations}
In this work, we propose an approach to explaining rare biomedical words for biomedical PTMs to help understand sentences with rare biomedical words. We conduct our experiments on the public biomedical datasets MedNLI and MedSTS with the authorization from the respective maintainers of the datasets. All experimental datasets involved have been de-identified by dataset providers and  only used for research.

==> _ACL Template-2/Table/case-study.tex <==
\begin{table*}[hptb]
\renewcommand{\arraystretch}{1.13}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c}
\hline
\hline
\multicolumn{1}{c|}{Sentence Pairs} & w/o paraphrases & w/ paraphrases \\ \midrule
\begin{tabular}[c]{@{}l@{}}P: She was found to have \textbf{BRBPR} \textit{(bright red blood per rectum)} on rectal exam. \\ H: the patient had bright red blood per rectum\end{tabular}     & Neutral  & \begin{tabular}[c]{@{}c@{}}Entailment\\ (\textbf{right answer})\end{tabular}    \\
\hline
\begin{tabular}[c]{@{}l@{}}P: Antenatal history - pregnancy complicated by chronic hypertension with increased \\ gestational hypertension leading to admission 3 days prior to delivery followed by cesarean\\ section.\\ H: The patient had \textbf{proteinuria} \textit{(The presence of protein in the urine)} during pregnancy\end{tabular} & Entailment      & \begin{tabular}[c]{@{}c@{}}Neutral\\ (\textbf{right answer})\end{tabular}        \\
\hline
\begin{tabular}[c]{@{}l@{}}P: Following this rehab admission she was sent to a different OSH on {[}**2725-10-26**{]}, \\ for acute \textbf{CHF} \textit{(congestive heart failure)} and at least one PEA arrest.\\ H: The patient has a poorly functioning heart.\end{tabular}                                                                 & Contradiction   & \begin{tabular}[c]{@{}c@{}}Entailment\\ (\textbf{right answer})\end{tabular}     \\
\hline
\hline
\begin{tabular}[c]{@{}l@{}}P: The patient was sent to the HD unit prior to coming to the floor for \textbf{workup} \textit{(A general}\\ \textit{medical examination to assess a persons health and fitness)} of fever.\\ H: The patient has an infection \end{tabular}                                                                 & \begin{tabular}[c]{@{}c@{}}Neutral\\ (\textbf{right answer})\end{tabular}    & Contradiction     \\
\hline
\begin{tabular}[c]{@{}l@{}}P: - \textbf{COPD} \textit{(chronic obstructive pulmonary disease)} - obesity - unspecified hypoxemia - \\CNS lymphoma c/b CVAs x3 (posterior circulation) and seizure d/o - history of SAH \\
while on coumadin - diastolic heart failure - coronary artery disease - atrial fibrillation -\\ hypertension - hyperlipidemia - severe OSA (did not tolerate CPAP in the past) - primary \\
hyperparathyroidism/25-vit D deficiency c/b nephrolithiasis - toxic multinodular \\
goiter with \textbf{subclinical} \textit{(Less than is needed for clinical reasons)} hyperthyroidism - \\ neovascular glaucoma c/b right eye blindness \\H: Patient has a history of malignancy \end{tabular}                                                                 & \begin{tabular}[c]{@{}c@{}}Neutral\\ (\textbf{right answer})\end{tabular}    & Entailment     \\
\hline
\hline
\end{tabular}
}
\caption[width=\textwidth]{Cases that model predicts differently after the supplement of paraphrases for rare biomedical words in MedNLI. ``P" for Premise and ``H" for Hypothesis. Words in \textbf{bold} are rare biomedical words and expressions in \textit{italic} inside the parentheses are the paraphrases of rare biomedical words.}
\label{case-study}
\end{table*}



==> _ACL Template-2/Table/few-shot.tex <==
\begin{table*}[h]
%\renewcommand{\arraystretch}{1.1}
\centering
\scalebox{0.8}{

\resizebox{\textwidth}{!}{
\begin{tabular}{r|ccccc}
% MedNLI
\hline
\hline
\multicolumn{6}{c}{MedNLI} \\

\hline
\diagbox{Model}{\#Samples} & 16 & 32 & 64 & 128 & 256\\
\hline
\multicolumn{1}{l|} {BERT-Large}  & 38.9 (3.7) & 44.5 (5.2) & 50.1 (5.2) & 54.8 (2.5) & 59.9 (1.2) \\
+ paraphrase & \textbf{40.8} (4.1) & \textbf{46.0} (5.5) & \textbf{53.3} (4.9) & \textbf{58.1} (1.4) & \textbf{61.9} (1.4) \\
\cdashline{2-6}
\textit{p}-value     & < 0.01 & 0.02 & < 0.01 & < 0.01 & < 0.01 \\

\hline

\multicolumn{1}{l|} {RoBERTa-Large} & 43.2 (6.7) & 52.1 (8.2) & 63.6 (4.6) & 69.2 (1.8) & 72.7 (1.4) \\
+ paraphrase & \textbf{49.5} (8.1) & \textbf{56.1} (7.6) & \textbf{65.6} (2.9) & \textbf{70.8} (0.7) & \textbf{74.0} (1.3) \\
\cdashline{2-6}
\textit{p}-value     & < 0.01 & 0.03 & 0.08 & 0.06 & 0.02 \\
\hline

\multicolumn{1}{l|} {BioBERT-Base} & 34.1 (1.5) & 38.5 (3.3) & 42.5 (4.6) & 52.1 (2.5) & 59.4 (1.6) \\
+ paraphrase & \textbf{36.3} (1.8) & \textbf{40.9} (3.5) & \textbf{45.2} (4.3) & \textbf{54.0} (2.3) & \textbf{60.4} (4.7) \\
\cdashline{2-6}
\textit{p}-value     & < 0.01 & < 0.01 & < 0.01 & 0.02 & 0.03 \\
\hline

\multicolumn{1}{l|} {PubMedBERT-Base} & 40.5 (3.4) & 46.8 (4.9) & 53.9 (4.0) & 62.9 (1.6) & 69.2 (1.1) \\
+ paraphrase & \textbf{45.0} (4.0) & \textbf{49.7} (5.0) & \textbf{56.4} (3.4) & \textbf{65.8} (1.6) & \textbf{71.0} (1.6) \\
\cdashline{2-6}
\textit{p}-value     & < 0.01 & < 0.01 & < 0.01 & < 0.01 & < 0.01 \\
\hline

\multicolumn{1}{l|} {SciBERT-Base} & 36.8 (1.2) & 41.4 (3.3) & 49.0 (3.7) & 54.7 (2.0) & 60.9 (1.0) \\
+ paraphrase & \textbf{38.2} (2.1) & \textbf{45.4} (5.2) & \textbf{50.1} (3.5) & \textbf{56.4} (2.2) & \textbf{61.9} (1.6) \\
\cdashline{2-6}
\textit{p}-value     & < 0.01 & 0.03 & 0.01 & 0.02 & < 0.01 \\
\hline

\multicolumn{1}{l|}{BC-RoBERTa-Large} & 51.3 (5.9) & 60.6 (6.7) & 71.0 (3.7) & 80.6 (1.3) & 83.1 (1.3) \\
+ paraphrase & \textbf{56.6} (5.0) & \textbf{62.3} (6.0) & \textbf{74.5} (3.0) & \textbf{81.1} (1.5) & \textbf{83.6} (1.0) \\
\cdashline{2-6}
\textit{p}-value     & < 0.01 & 0.05 & < 0.01 & 0.02 & 0.01 \\

\hline
\hline
\end{tabular}}}
\caption{
Few-shot results on the MedNLI task using various pre-trained models with training and development sets of different sizes. We report mean (standard deviation) performance of accuracy over 10 different random seeds, along with the \textit{p}-value of the paired \textit{t}-test. + paraphrase: with paraphrases of selected rare biomedical words.}
\label{few-shot-task-mednli}

\end{table*}

\begin{table*}[h!]
\renewcommand{\arraystretch}{1.05}
\centering
\scalebox{0.8}{

\resizebox{\textwidth}{!}{
\begin{tabular}{r|ccccc}
\hline
\hline
%MedSTS-2018
\multicolumn{6}{c}{MedSTS} \\
\hline
\diagbox{Model}{\#Samples} & 16 & 32 & 64 & 128 & 256\\
\hline
\multicolumn{1}{l|} {BERT-Large} & 14.1 (7.4) & 24.8 (10.1) & 43.6 (5.7) & 60.2 (4.7) & 72.2 (4.5) \\
+ paraphrase & \textbf{18.5} (9.0) & \textbf{28.2} (12.1) & \textbf{48.7} (7.1) & \textbf{64.1} (5.1) & \textbf{72.7} (4.6) \\
\cdashline{2-6}
\textit{p}-value     & < 0.01 & 0.04 & < 0.01 & 0.01 & 0.08 \\
\hline

\multicolumn{1}{l|} {RoBERTa-Large} & 29.5 (9.3) & 41.7 (18.5) & 55.1 (12.1) & 67.6 (6.8) & 76.0 (3.5) \\
+ paraphrase & \textbf{34.6} (13.5) & \textbf{46.1} (13.0) & \textbf{57.7} (12.7) & \textbf{69.9} (6.7) & \textbf{77.2} (3.7) \\
\cdashline{2-6}
\textit{p}-value     & 0.04 & 0.01 & 0.02 & 0.03 & 0.02\\
\hline

\multicolumn{1}{l|} {BioBERT-Base} & 17.3 (14.4) & 26.3 (13.7) & 41.4 (9.0) & 52.2 (10.6) & 63.0 (7.3) \\
+ paraphrase & \textbf{20.0} (12.9) & \textbf{28.2} (12.8) & \textbf{43.1} (8.6) & \textbf{53.7} (9.2) & \textbf{64.2} (7.1) \\
\cdashline{2-6}
\textit{p}-value     & 0.03 & 0.02 & 0.01 & 0.02 & 0.02 \\
\hline

\multicolumn{1}{l|} {PubMedBERT-Base} & 10.3 (9.8) & 22.8 (10.7) & 36.9 (10.6) & 48.1 (11.9) & \textbf{65.5} (9.5) \\
+ paraphrase & \textbf{18.8} (13.7) & \textbf{27.3} (11.6) & \textbf{39.9} (10.4) & \textbf{49.4} (12.4) & 65.1 (9.4) \\
\cdashline{2-6}
\textit{p}-value     & 0.04 & 0.01 & < 0.01 & 0.07 & 0.1 \\
\hline

\multicolumn{1}{l|} {SciBERT-Base} & 15.2 (16.9) & 29.1 (18.2) & 45.5 (14.0) & 60.8 (9.0) & 72.2 (7.3) \\
+ paraphrase & \textbf{19.2} (15.5) & \textbf{32.6} (18.4) & \textbf{48.9} (14.4) & \textbf{62.5} (8.3) & \textbf{73.4} (6.8) \\
\cdashline{2-6}
\textit{p}-value     & 0.01 & < 0.01 & 0.02 & < 0.01 & < 0.01 \\
\hline
\multicolumn{1}{l|} {BC-RoBERTa-Large} & \textbf{54.2} (8.1) & 63.9 (9.2) & 73.3 (3.8) & 77.4 (2.7) & 81.5 (1.5) \\
+ paraphrase & 53.0 (7.4) & \textbf{67.2} (6.6) & \textbf{74.5} (2.7) & \textbf{79.1} (1.6) & \textbf{81.8} (1.2) \\
\cdashline{2-6}
\textit{p}-value     & 0.08 & 0.01 & 0.03 & < 0.01 & 0.02 \\
\hline
\hline
\end{tabular}}}
\caption{
Few-shot results on the MedSTS task using various pre-trained models with training and development sets of different sizes. We report mean (standard deviation) performance of Pearson correlation coefficient over 10 different random seeds, along with the \textit{p}-value of the paired \textit{t}-test. + paraphrase: with paraphrases of selected rare biomedical words.}
\label{few-shot-task-sts}

\end{table*}




==> _ACL Template-2/Table/more-data-mednli.tex <==
\begin{table*}[htbp]
%\renewcommand{\arraystretch}{1.1}
\centering
\scalebox{0.9}{
\begin{tabular}{r|cccccc}
\hline
\hline
\multicolumn{7}{c}{MedNLI} \\
\hline 
\diagbox{Model}{\#Training} & 512 & 1024 & 2048 & 4096 & 8192 & full-size \\
\hline
BC-RoBERTa-Large & 84.8 (0.7) & 85.5 (0.8) & 86.4 (0.5)&86.3 (0.7)& 86.2 (0.6) & 85.9 (0.6)\\
+ paraphrases & \textbf{85.2} (0.8) &\textbf{86.3} (1.0) & 86.4 (0.7)& 86.3 (0.6)&\textbf{86.7} (0.5) & \textbf{86.7} (0.7)\\
\cdashline{2-7}
\textit{p}-value     & 0.05 & < 0.01 & 0.43 & 0.36 & < 0.01 & 0.02 \\
\hline
\hline
\end{tabular}}
\caption{
Test results on the MedNLI dataset with larger size of training sets. We report mean (and standard deviation) accuracy. + paraphrase: with paraphrases of rare biomedical words.
}
\label{mednli-more}
\end{table*}

==> _ACL Template-2/Table/number_of_rare_word.tex <==
\begin{table*}[tb]
\centering
%\renewcommand{\arraystretch}{1.1}
%\scalebox{0.9}{
\resizebox{\textwidth}{!}
{%
\begin{tabular}{cc|cccccccccc|c}
\hline
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\diagbox{threshold}{Dataset}}}&  \multicolumn{2}{c}{16}  & \multicolumn{2}{c}{32} & \multicolumn{2}{c}{64} & \multicolumn{2}{c}{128} & \multicolumn{2}{c|}{256} & \multicolumn{1}{c}{\multirow{2}{*}{Test}}\\
\cline{3-12}
\multicolumn{2}{c|}{\multirow{2}{*}{}}& Train & Dev & Train & Dev & Train & Dev & Train & Dev &  Train & Dev & \multicolumn{1}{c}{\multirow{2}{*}{}} \\
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textit{t} = 20k}}& *&1.1  & 1.1  & 1.9  & 1.7   & 3.4  & 3.9  & 6.8  & 7.6  & 13.2 & 14.3 & 29  \\
\cline{2-13}
\multicolumn{1}{c|}{}& **& 1.1 &1.1 &1.9 &1.8  &3.7 &4.4 &7.3 &9.0 &16.3 &21.1 &129 \\
\hline

\multicolumn{1}{c|}{\multirow{2}{*}{\textit{t} = 50k}}&* &1.8 &1.5  &3.5 &2.2  &6.8&4.8  &12.4 &9.2 &21.8&17.0 & 40\\
\cline{2-13}
\multicolumn{1}{c|}{} & ** &1.8&1.5 &3.5&2.3 &7.1&5.4 &13.1&11.2 &26.6&24.9& 196\\
\hline

\multicolumn{1}{c|}{\multirow{2}{*}{\textit{t} = 100k}}&* &1.8&1.6&3.8&2.6&7.2&5.9&14.0&11.1&25.3&20.2&41\\
\cline{2-13}
\multicolumn{1}{c|}{} & ** &1.8&1.6&3.8&2.8&7.6&6.5&14.8&13.0&30.8&25.4&179\\
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textit{t} = 200k}}&* &1.9&2.1&4.3&3.5&7.6&6.8&13.9&12.3&23.3&21.7&41\\
\cline{2-13}
\multicolumn{1}{c|}{} & ** &1.9&2.1&4.3&3.7&8.2&7.8&15.3&15.5&33.4&32.6&185\\

\hline
\hline
\end{tabular}
}
\caption{The number of selected rare biomedical words in the training, development and test sets for different few-shot datasets on MedNLI.  ``\textit{t} = 20k'' means the threshold for rare biomedical words is 20k. ``*'' is the number of different rare biomedical words within the threshold. ``**'' denotes the total occurrences of rare biomedical words in the dataset (a rare biomedical word can appear more than once).}
\label{number_of_rare_word}
\end{table*}

==> _ACL Template-2/Table/only-test.tex <==
\begin{table}[H]
%\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}
{%
\begin{tabular}{c|ccccc}
\hline
\hline
\#Samples& 16 & 32 & 64 & 128 & 256 \\
\hline
w/o p-       & 51.3 & 60.6 & 71.0 & 80.6 & 83.1 \\
w/ p-train\&dev   & 49.5 & 56.9 & 62.5 & 76.5 & 82.1 \\
w/ p-test & & & & & \\
w/ p-all & 56.6 & 62.3 & 74.5 & 81.1 & \textbf{83.6} \\
\hline
\hline
\end{tabular}%
}
\caption{Results for few-shot learning through different paraphrasing strategy on MedNLI with the BC-RoBERTa-Large model. w/o p-: without paraphrases for rare biomedical words. w/ paraphrase\dag: with paraphrases for rare biomedical words in test sets. w/ paraphrase: with paraphrases for rare biomedical words in all sets.}
\label{table-only-test}
\end{table}



==> _ACL Template-2/Table/threshold.tex <==
\begin{table}[htbp]
%\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}
{%
\begin{tabular}{c|ccccc}
\hline
\hline
\#Samples& 16 & 32 & 64 & 128 & 256 \\
\hline
\textit{w/o} paraphrase       & 51.3 & 60.6 & 71.0 & 80.6 & 83.1 \\
\textit{t} = 20k & 55.0 & 61.9 & 72.4 & 80.6 & 83.4 \\
\textit{t} = 50k & 54.2 & 62.1 & 73.8 & 81.0 & \textbf{83.7} \\
\textit{t} = 100k & 54.5 & \textbf{62.4} & 73.4 & 80.4 & 83.2 \\
\textit{t} = 200k & \textbf{56.6} & 62.3 & \textbf{74.5} & \textbf{81.1} & 83.6 \\

\hline
\hline
\end{tabular}%
}
\caption{Results for few-shot learning with different thresholds of rare biomedical words on MedNLI with the BC-RoBERTa-Large model. \textit{w/o} paraphrase: without paraphrases for rare biomedical words. \textit{t}: the threshold for rare biomedical words.}
\label{table-threshold}
\end{table}




==> _ACL Template-2/Text/0.Abstract.tex <==
\begin{abstract}

Prompt-based fine-tuning for pre-trained models has proven effective for many natural language processing tasks under few-shot settings in general domain. However, tuning with prompt in biomedical domain has not been investigated thoroughly. Biomedical words are often rare in general domain, but quite ubiquitous in biomedical contexts, which dramatically deteriorates the performance of pre-trained models on downstream biomedical applications even after fine-tuning, especially in low-resource scenarios. We propose a simple yet effective approach to helping models learn rare biomedical words during tuning with prompt. Experimental results show that our method can achieve up to 6\% improvement in biomedical natural language inference task without any extra parameters or training steps using few-shot vanilla prompt settings.
%Rare biomedical words, which are quite ubiquitous in biomedical contexts, can affect the performance of pre-trained models, especially in low-resource scenarios.
\end{abstract}




==> _ACL Template-2/Text/1.introduction.tex <==
\section{Introduction}
%可以加一段论述类比人类阅读文献时查字典的行为
%Understanding key concept is fundamental to most biomedical text understanding tasks. Those key concepts are usually composed of professional and rare terms. For instance, XXXX. To this end, people usually refer to professional dictionaries and biomedical knowledge bases. However, NLP models still have a huge gap in terms of both versatile reading and knowledgeable learning compared to human learners. Therefore, it is a valuable problem to empower machine reading systems to better understand domain-specific concepts.

%第一段就可以直入主题，预训练模型在通用域取得了巨大的成功，成为了一种新的范式。所以在医学领域上也出现了不少的尝试。但是由于医学领域的自身挑战使得预训练模型在医学领域表现平平。
Pre-trained models have achieved a great success in natural language processing (NLP) and become a new paradigm for various tasks~\citep{peters2018deep,devlin2019bert,liu2019roberta,qiu2020pre}. Many studies have paid attention to pre-trained models in biomedical NLP tasks~\citep{lee2020biobert,lewis2020pretrained,zhao2021recent}. However, plain pre-trained models sometimes cannot do very well in biomedical NLP tasks. % due to the differences between biomedical texts. 
%第二段介绍医学领域上的两个挑战，数据少和稀疏词多。分别论述两个挑战，带例子。
In general, there are two challenges to fully exploit the potential of the pre-trained models for biomedical NLP tasks, i.e., (1) \textbf{limited data} and (2) \textbf{rare biomedical words}.
Firstly, it is common that the amount of biomedical labeled data is limited due to strict privacy policy constraints~\citep{vsuster2017short}, high cost and professional requirement for data annotation.
Pre-trained models perform poorly with few samples since abundant training samples are essential to optimize task-related parameters~\citep{liu2021pre}.
Secondly, biomedical words are usually low-frequency words but critical to understanding biomedical texts.
As an example of natural language inference (NLI) task in Figure~\ref{wrong-case}, the model goes wrong during tuning when faced with a rare word ``\textit{afebrile}''\footnote{There are around 4 billion words in the selected biomedical pre-training texts while ``afebrile'' appears only about 100,000 times, accounting for 0.0025\%.}
%For comparison, the frequency of ``fever'' is 5 times that of ``afebrile''.}}'' 
in the premise, whose meaning is ``\textit{having no fever}''. It can be no easy for the pre-trained models to predict the correct label if the models haven't seen the rare biomedical words for enough times during pre-training or tuning stage. Thus, pre-trained models cannot capture the precise semantics of biomedical texts in the scenario of low-resource tasks.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{Figure/wrong-case-220430}
    \caption{Failures of a biomedical pre-trained model~\citep{lewis2020pretrained} on the biomedical NLI task.}
    \label{wrong-case}
\end{figure*}

%第三段，写一下prompt 技术的设计初衷和相关工作。因此可以被引入到医学预训练模型上来解决few-shot问题。

With very few annotated samples available for a new task, it is hard to effectively fine-tune pre-trained models with the additional task-specific parameters, which is even more of a challenge to biomedical domain as mentioned above. Prompt technique has been introduced to smooth the fine-tuning process in the few-shot settings by narrowing down the gap between pre-training stage and the downstream task in general domain~\citep{liu2021pre}, as demonstrated in Figure~\ref{intro_prompt}. Therefore, it is beneficial to adapt prompt-based tuning to biomedical NLP tasks.%``pre-training, prompt and predicting'' framework to biomedical NLP tasks.


%downstream task inherits task paradigm from pre-training instead of training additional task-related layers. % Thus, downstream tasks wouldn't be a far cry from the pre-training tasks, which empowers the PTMs to perform better in the case of restricted amount of data.


%Promising results gained by ``Pre-training and Fine-tuning'' model are on the basis of sufficient training steps of additional parameters pertaining to new tasks, such as BERT~\citep{devlin2019bert}. Otherwise, PTMs are unlikely to perform well in few-shot settings~\citep{moradi2021gpt}.

%With limited tuning data for a new task, it is hard to fine-tune the PTMs and the new task-specific parameters effectively. To solve the above problem, ``Pre-training, Prompt and Predicting'' is proposed to . 
% transfer to medical


%第四段，但是影响医学与训练模型的第二个挑战还很少有研究。因此，本文提出融合promot或者说基于prompt的医学概念解释方法来解决第二个挑战。论述下方法好在哪。
Although the challenge of rare words is a critical problem for the biomedical pre-trained models, only a handful of works have studied the issue and most of them focus on enriching the representation of rare words through pre-training stage~\citep{schick2020rare,yu2021dict,wu2020taking}.
Thus, it naturally requires them to involve a second-round pre-training or further training steps with biomedical knowledge to achieve the above goal, which is highly time-consuming and inefficient. Alternatively, we emphasize on tuning stage instead of pre-training to resolve these issues. When coming across an unknown word, human may seek the dictionary for its paraphrase. Enlightened by this phenomenon, we propose to explain rare biomedical words with the paraphrases on the basis of prompt-based tuning. The new approach could enhance tuning capability in understanding biomedical words. Furthermore, as a generic plug-in module for non-specific datasets, our approach is model-agnostic and can be easily transferred to other domains.\footnote{We release our code at \url{https://github.com/s65b40/prompt\_n\_paraphrase}}

% build upon the recent success of prompt and help biomedical PTMs understand biomedical terms in the downstream tasks during tuning with prompt by looking them up in the dictionary, which mimics the behavior when human reads as knowledge enhancement. We attach the paraphrases of selected biomedical rare words to the words themselves in the datasets of downstream tasks only during tuning stage  without extra pre-training. Also, our method is a plug-in module for task datasets and model-agnostic, which can be easily transferred to other domains and models\footnote{We plan to release our code at ...}.


%And if a trained model comes across new rare words in another task, extra pre-training will be inevitable.
%leverage non-rare tokens to approximate rare words~\citep{schick2020rare} or inject knowledge of certain set of rare words into pre-training procedure to ~\citep{yu2021dict,wu2020taking}. 


%Notable works alleviate this problem via leveraging non-rare words or tokens to approximate rare words~\citep{schick2020rare} or injecting knowledge or contexts of certain set of rare words into pre-training procedure to enrich the representation of rare words~\citep{yu2021dict,wu2020taking}. 

%第五段，实验结论论述    
% Also, words are generally in long-tail distribution and \citet{schick2020rare,wu2020taking} have discussed that rare words hinder the PTMs to understand sentences correctly. biomedical rare words, which are semantically more related to biomedical tasks, tend to barrier the biomedical PTMs more. 
In summary, our contributions are as follows:
\begin{itemize}
    \item We investigate a valuable problem of the adaptation of pre-trained models to few-shot scenarios to enhance biomedical text understanding with a focus on rare biomedical words.
    \item We propose a novel method to combine the prompt paradigm and paraphrases of rare biomedical words in the tuning stage of pre-trained models to address the limitation caused by ``rare but key words'' in biomedical texts.
    \item We evaluate on six pre-trained models over two biomedical natural language understanding datasets$-$MedNLI and MedSTS. Our approach can improve the performance by up to 6\% in the few-shot settings. Moreover, we discuss how the paraphrases improve the pre-trained models and provide a perspective about task-related rare words.
\end{itemize}

%\item We combine the prompt-based fine-tuning and a portable plug-in module to help understand biomedical rare words. Afterwards,

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figure/intro-prompt-1905.pdf}
    \caption{Examples for paradigms of (a) Masked Language Model (MLM) pre-training; (b) Task-specific fine-tuning; (c) Prompt-based fine-tuning, with same task as pre-training process; (d) Paraphrase-enhanced prompt-based fine-tuning. Best viewed in color.}
    \label{intro_prompt}
\end{figure*}





==> _ACL Template-2/Text/2.RelatedWork.tex <==
\section{Related Work}
\paragraph{Representation learning of rare words in pre-trained models.}
Words in the vocabulary list follow a Zipf distribution~\citep{zipf2016human} by and large. Previous works have shown that the word representation space of the pre-trained models is anisotropic and high-frequency words dominate the representation of a sentence which can induce semantic bias~\citep{gao2018representation,li-etal-2020-sentence,yan-etal-2021-consert}. Meanwhile, it has also been proven that rare words limit the performance of pre-trained models as the rare words can play a decisive role in the sentence understanding~\citep{schick2020rare,wu2020taking,yu2021dict}. \citet{schick2020rare} introduced one-token approximation to infer the embedding of arbitrary rare word by a single token. \citet{wu2020taking} proposed to take notes on the fly to maintain a note dictionary for rare words to save the contextual information that helps enhance the representation during pre-training.


\paragraph{Biomedical pre-trained models.}
With the booming trend of pre-trained models in NLP tasks~\citep{peters2018deep,devlin2019bert,liu2019roberta}, various trials have been made to investigate the pre-trained models in biomedical domain~\citep{peng2019transfer,lee2020biobert,huang2019clinicalbert}. %by pre-training on biomedical texts.
\citet{lewis2020pretrained} and \citet{gu2021domain} further built the domain-specific vocabulary to amend the representation of biomedical words. More recent works guided biomedical pre-trained models with domain knowledge. For example, \citet{zhang2021smedbert} amplified the biomedical entities with type information from neighbor entities. \citet{michalopoulos2021umlsbert} learned clinical word embeddings with the association of synonyms in the Unified Medical Language System (UMLS) Metathesaurus. 

\paragraph{Tuning pre-trained models with prompt.}
Many works were dedicated to applying prompt in fine-tuning by adapting the downstream tasks to the paradigm of pre-training tasks. Prompts that have been employed by now can be categorized into two groups: (1) discrete prompt in natural language~\citep{schick2021exploiting, gao-etal-2021-making} and (2) continuous prompt in representation based on trainable vectors~\citep{li-liang-2021-prefix,shin2020eliciting}. Discrete prompt follows the settings of pre-training tasks and converts the downstream tasks into a cloze question format without requiring additional parameters. Continuous prompt inserts prompt embeddings into the models, which could perform better than discrete prompt but at the expense of explainability and extra training cost on additional data for the prompt embeddings~\citep{wei2021finetuned, gu2021ppt}. Recently, \citet{liu2021p} considered training continuous prompts as a parameter-efficient method instead of tuning the parameters of the entire pre-trained model. In this study, we follow the paradigm of discrete prompt to avoid introducing more ambiguity from the prompt embeddings or training costs on additional training data.

==> _ACL Template-2/Text/3.RareMedicalWordsandParaphrases.tex <==
\section{Method}
% \section{Rare Biomedical Words and Paraphrases}
In this section, we introduce how we find the rare biomedical words and append paraphrases to the rare biomedical words with the prompt-based tuning of pre-trained models in a model-agnostic plug-in manner. 

\subsection{Rare Words}
The rarity of a word mostly depends on its frequency in a certain corpus, which can vary from context to context. A rare word in the pre-training corpora is possibly not \textit{that} rare in the down-stream tasks. In this work, we define the ``rare words'' as the words whose frequency is under a specific threshold in the pre-training corpora as aforementioned. 

Meanwhile, although the pre-trained models tokenize the input words into tokens, tokenizers based on byte-pair encoding~\citep{sennrich2016neural} or WordPiece~\citep{6289079} split words into sub-words by frequency or likelihood, which is both dominated by the common words. Thus, although the rare words can be split into possible non-rare tokens, there is not much semantics from the original rare words retained after being tokenized into common tokens for the pre-trained models. Also, tokenizers of different pre-trained models can tokenize the same rare word into different tokens and consequentially make rare tokens model-related. For example, BERT-Large~\citep{devlin2019bert} model tokenizes ``\textit{afebrile}'' into ``\textit{af-eb-ril-e}'' while Biomedical-Clinical-RoBERTa-Large~\citep{lewis2020pretrained} model tokenizes it into ``\textit{a-fe-brile}''. 


\subsection{Selection of Rare Biomedical Words}
\label{bc-roberta}
To obtain the frequency of words, we adopt the biomedical corpora including PubMed abstract,\footnote{\url{https://pubmed.ncbi.nlm.nih.gov}} PubMed Central\footnote{\url{https://www.ncbi.nlm.nih.gov/pmc}} (PMC) full-text and MIMIC-III dataset,\footnote{\url{https://physionet.org/content/mimiciii/1.4/}} which are widely used for pre-training biomedical language models, such as BC-RoBETRa~\citep{lewis2020pretrained}, BioBERT~\cite{lee2020biobert}, and PuBMedBERT~\cite{pubmedbert}. We loop the above corpora to obtain the frequency of each word in the pre-training phase. The rare words found in biomedical corpora are likely to contain words not only in the biomedical domain but also in the general domain. Instead of including all rare words, we consider rare words from biomedical domain with the following two reasons:
(1) \textbf{Domain-specific distribution}: unlike the general domain,  distribution of words in the biomedical domain is shaped with domain-specific terms, such as disease, medicine, diagnosis and treatment~\citep{lee2020biobert}. %Word distribution in general domain differs from that in biomedical domain~\citep{lee2020biobert}. Biomedical terms, such as disease, medicine, diagnosis and treatment are ubiquitous in biomedical domain but less common in general domain.% 
(2) \textbf{Task-specific words}: rare words from the biomedical domain can contribute more to biomedical tasks than that from the general domain. Therefore, we introduce a threshold, an empirical hyper-parameter, to assist the selection of rare words following~\citet{yu2021dict}, and we also experiment with different thresholds for the rare words in Section~\ref{threshold}. We retrieve the paraphrases of the rare biomedical words from an online dictionary ``Wiktionary''.\footnote{Wiktionary - \url{https://en.wiktionary.org/}} To optimize the selection, we only keep the rare words that are tagged with medical-related categories from the Wiktionary, i.e. \textit{medical}, \textit{medicine}, \textit{disease}, \textit{symptom} and \textit{pharmacology}.


%Afterwards, with the help of an online dictionary - Wiktionary\footnote{\url{https://en.wiktionary.org/}}, we retrieve the paraphrases of rare words along with the category labels. Only rare words with medical-related labels, i.e. ``medical'', ``medicine'', ``disease'', ``symptom'',``pharma-'', are reserved as rare biomedical words since the semantics of biomedical rare words can be more related to biomedical tasks.
% Biomedical rare words can be more valuable than general rare words to biomedical tasks. To obtain rare words, we set a threshold on the word frequency in the pre-training corpora empirically as a hyper-parameter similar to~\citet{yu2021dict}. 

\subsection{Selection of Paraphrases}
\label{selection_paraphrase}
There can be more than just one paraphrase for a rare biomedical word and it is tricky to choose the most appropriate paraphrases. Therefore, to avoid introducing noise from the inappropriate paraphrases, we exclude rare biomedical words with more than one corresponding paraphrase. In addition, we ignore paraphrases that contain additional rare words whose frequencies are below the set threshold since it only replaces one rare word with another. Meanwhile, considering that biomedical abbreviations are likely to be tokenized into separate letters with no meaningful semantic information, we retrieve and append the paraphrases to all the biomedical abbreviations. 

\subsection{Prompt-based Fine-Tuning with Paraphrases}
When coming across new words during reading, humans habitually seek dictionaries for the corresponding paraphrases to help us understand. Following the same idea, we guide the pre-trained models with paraphrases, where rare words are followed by the parenthesis punctuation, as shown in Figure~\ref{intro_prompt}(d). In this way, given a pre-trained model, paraphrases of biomedical rare words can be considered as a portable plug-in module and generated for any dataset instantly before prompt-based fine-tuning. 
% We adopt the settings of prompt template and verbalizers from~\citet{schick2021s} and~\citet{gao-etal-2021-making} for our method is prompt-agnostic.% and prompt in natural language can offer more interpretability as well.

==> _ACL Template-2/Text/4.Experiments.tex <==
% experiment results 
\section{Experiments}

\subsection{Setup}
\paragraph{Models.} 
To demonstrate that our approach is model-agnostic, we adopt six pre-trained models in both general and biomedical domains, namely (1) BERT-Large~\citep{devlin2019bert}, (2) RoBERTa-Large~\citep{liu2019roberta}, (3) BioBERT-Base~\citep{lee2020biobert}, (4) PubMedBERT-Base~\citep{pubmedbert}, (5) SciBERT-Base~\citep{beltagy-etal-2019-scibert} and (6) BC-RoBERTa-Large (Biomedical-Clinical RoBERTa-Large)~\citep{lewis2020pretrained}. During prompt-based tuning, we use the same set of hyper-parameters for all the six pre-trained models, including learning rate of $1 \times 10^{-5}$, batch size of 2 and max epoch of 10.

\paragraph{Datasets.}  Previous work demonstrates that rare words have more impact on Natural Language Understanding (NLU) tasks than Information Extraction (IE)~\citep{schick2020rare}, while most biomedical NLP tasks fall into the category of IE~\citep{shin2020bio,gu2021domain}. To better demonstrate the method effectiveness, we perform evaluation over the two biomedical NLU datasets, namely MedNLI~\citep{romanov2018lessons} and MedSTS\footnote{We use ClinicalSTS-2018 which is a sub-dataset of MedSTS provided by the maintainers of the MedSTS project.}~\citep{wang2020medsts}.

% Note that rare words hinder the performance of pre-trained models more in natural language understanding (NLU)~\citep{schick2020rare} than in other NLP tasks. However, most biomedical and clinical NLP tasks fall in the category of information extraction~\citep{shin2020bio,gu2021domain}. Thus, we evaluate our method over two NLU-relevant biomedical tasks - MedNLI~\citep{romanov2018lessons} and MedSTS\footnote{We use ClinicalSTS-2018 which is a sub-dataset of MedSTS provided by the maintainers of MedSTS project.}~\citep{wang2020medsts}. 

MedNLI is a natural language inference dataset where premises are selected from real clinical notes in MIMIC-III~\citep{johnson2016mimic}. And MedSTS is a semantic textual similarity dataset gathered from a clinical corpus at Mayo Clinic and the ground-truth label of the similarity is the mean of the subjectively annotated scores from multiple annotators. As MedSTS is actually a regression task, we adapt the task following~\citet{gao-etal-2021-making} and convert it into a classification task. We use the same data splitting of training, development and test sets as the original two datasets. Statistics of datasets can be found in Table~\ref{data_stat}.  

\begingroup
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{table}[H]
\centering
\scalebox{0.7}{
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc}
\hline
\hline
\textbf{Dataset}                  & \textbf{Train} & \textbf{Dev}  & \textbf{Test} \\ \hline
MedNLI & 11,232 & 1,395 & 1,422 \\
\hline
MedSTS & 750   & /    & 318  \\ \hline \hline
\end{tabular}%
}}
\caption{Statistics of the MedNLI and MedSTS datasets. We use the ClinicalSTS-2018 subset of MedSTS.}
\label{data_stat}
\end{table}
\endgroup

\paragraph{Few-shot datasets.} 
Initialized with 10 different random seeds, we randomly sample instances within the range of 16 to 256 from corresponding training and development sets as the few-shot training and development sets. The original test set is directly used as the few-shot test set. Note that there is no development set in MedSTS, so we sample the few-shot development set from the original training set with the same quantity of samples as the few-shot training set with no overlapping instances. Accuracy and Pearson correlation coefficients are used as the evaluation metrics for MedNLI and MedSTS, respectively.



\paragraph{Prompt settings.} 
We prepare discrete prompts using the same prompt settings from~\citet{schick2021exploiting} and~\citet{gao-etal-2021-making}, which correspond to the NLI and STS tasks respectively in Table~\ref{prompt}.% to verify the effectiveness of paraphrases of biomedical rare words rather than the prompt template.
% Since the selection of discrete prompt template is not the key point of our work and our method is template-agnostic, we just combine the prompt settings from~\citet{schick2021exploiting} and~\citet{gao-etal-2021-making} for the natural language inference and semantic textual similarity tasks empirically without further adaption in Table~\ref{prompt} to verify the effectiveness of paraphrases of biomedical rare words rather than the prompt template.

\begin{table}[H]
\renewcommand{\arraystretch}{1.2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c}
\hline
\hline
\textbf{Task} & \textbf{Template}                                          & \textbf{Verbalizer} \\
\hline
MedNLI        & \textless{}Sent1\textgreater{}. {[}MASK{]}. \textless{}Sent2\textgreater{} & Yes/No/maybe           \\
MedSTS        & \textless{}Sent1\textgreater{}. {[}MASK{]}. \textless{}Sent2\textgreater{} & Yes/No    \\
\hline
\hline
\end{tabular}%
}
\caption{Prompt settings for MedNLI and MedSTS.}
\label{prompt}
\end{table}

\paragraph{Rare biomedical words and paraphrases.}
We find that a threshold of rare biomedical words at 200,000, corresponding to a frequency less than 0.005\% in the pre-training corpora, can yield better results in most scenarios % with the Biomedical and Clinical RoBERTa-large~\citep{lewis2020pretrained} model 
(details in Section~\ref{threshold}), so we consider the biomedical words that appear less than 200,000 times as ``rare biomedical words'' and prepare the same rare word and paraphrase sets for all the models to validate the generalization ability of our approach. % Paraphrases of those rare words, where there is no other rare biomedical word within, are attached to the rare words.

\subsection{Few-shot learning results}
We report the mean accuracy for the MedNLI task and Pearson correlation coefficient for the MedSTS task over 10 sampled few-shot datasets based on different random seeds, along with standard deviation and \textit{p}-value of paired \textit{t}-test. Table~\ref{few-shot-task-mednli} and Table~\ref{few-shot-task-sts} show the results for the two tasks on six pre-trained models.

\paragraph{Results on MedNLI.} 
The pre-trained models with the paraphrases for rare biomedical words can outperform the baselines in all cases and can bring about 6\% improvement on average for few-shot learning with 16 training samples and 2\% with 256 training samples. All performance improvements are statistically significant with \textit{p}-value less than 0.05 except only two out of ten cases from the RoBERTa-based model in general domain. %It indicates that the paraphrases of rare biomedical words are possibly not as helpful in general domain for the models that are not pre-trained with biomedical texts. 
Besides, small pre-trained biomedical models are comparable with large pre-trained models in the general domain under the few-shot settings. Furthermore, with more training samples up to 256, our approach is consistently effective.
%small-scale models pre-trained on biomedical texts is sometimes inferior to large-scale models pre-trained on general domain for the MedNLI task in the few-shot settings. Meanwhile, with more training samples up to 256, our approach is consistently effective.

\paragraph{Results on MedSTS.} 
Similar to MedNLI, the incorporation of paraphrases improves the performances compared with baselines in general. For some cases, statistical significance is not as stable as that on MedNLI for two reasons: 
 (1) Some ground-truth labels in the MedSTS task can be biased due to the subjectivity of annotation~\citep{yang2020measurement}; % Semantic textual similarity task is a regression task where gold label is annotated subjectively and therefore can be biased. 
 (2) Rare biomedical words shared in the sentence pair of the same sample can be a shortcut for the pre-trained models, as the paraphrases increase the overlap between the two sentences and mislead the models to overlook the rest of the sentences~\citep{mccoy2019right}.
%There can be same rare biomedical words in both sentences within a sample, leading to more overlaps between the two sentences with paraphrases introduced above, which can be a shortcut learned by the pre-trained models and affects the model performance~\citep{mccoy2019right}. 
 %(3) Pearson correlation co-efficiency enables results of few-shot learning with more fluctuations than the accuracy metric. % As we use Pearson correlation coefficient as the evaluation metrics, the results can fluctuate more than using accuracy, especially in few-shot scenarios. % Similarly, large pre-trained models in the general domain perform better than the small pre-trained biomedical models. Pearson correlation co-efficiency f

\input{Table/few-shot}

\subsection{Thresholds for rare biomedical words}
\label{threshold}
The number of paraphrases of rare biomedical words involved in the samples can directly affect the model performance, which is controlled by the pre-set threshold.
%The quantity of rare biomedical words and paraphrase involved in the training samples can significantly affect model performance and is correlated with the threshold of rare biomedical words we set. 
To measure the influence of different thresholds, we conduct experiments over MedNLI task since its labelled data is more objective compared to MedSTS. 
% And as natural language inference is an objective classification task while semantic textual similarity is a regression task with gold label based on relatively subjective annotation, we explore the effect of the thresholds of rare biomedical words with MedNLI task. 


\paragraph{Statistics of rare biomedical words.}
Table~\ref{number_of_rare_word} shows the mean of rare biomedical words in the training, development and test sets under different thresholds for the MedNLI task. % Firstly, we cut the number of rare biomedical words inside the training, development and test sets in the few-shot datasets to different thresholds in Table~\ref{number_of_rare_word} on MedNLI task. 
Among the above thresholds, the number of rare biomedical words varies from 29 to 41 in the test set, while the total number of all rare biomedical words varies from 129 to 196. Each rare biomedical word appears around 5 times on average in the test set.  %There are from 29 to 41 unique rare biomedical words selected in the full-size test set with different thresholds. 
% From 129 to 196 rare biomedical words are attached with their paraphrases in total and a rare word appears around 5 times in the test set on average. 
%With the increase of the threshold, the number of rare biomedical words grows while the overall paraphrases may break the increase due to the filter of paraphrases (see Section~\ref{selection_paraphrase}).
Note that as the threshold increases, the number of paraphrases does not necessarily increase as fast as the number of rare biomedical words which is because that although higher threshold does include more rare biomedical words, not all are appended with paraphrases as some of them are excluded as mentioned in Section~\ref{selection_paraphrase}.
%Note that as the threshold increases, although the number of total rare biomedical words under the threshold increases, the number of paraphrases appended in the may not increase because some paraphrases can be eliminated as introduced in Section~\ref{selection_paraphrase}.
\input{Table/number_of_rare_word}

% \paragraph{Performance with different thresholds}
In addition to the fixed threshold of 200,000, we experiment with the thresholds ranging from 20,000 to 200,000. Table~\ref{table-threshold} further demonstrates the effectiveness of paraphrases of rare biomedical words in most cases, where 200,000 of the threshold performs the best.\footnote{We also attempt with thresholds higher than 200,000 but it will not bring improvement as much as 200,000.} %It demonstrates that the paraphrases of rare biomedical words can enhance the pre-trained model performance for most scenarios with different thresholds of rare words in Table~\ref{table-threshold} and with the threshold of 200,000 the model performs better generally. 


\input{Table/threshold}


% \subsection{Main Results and Analysis}
%We report average accuracy for MedNLI and pearson correlation coefficient for MedSTS along with standard deviation. Table~\ref{few-shot-task} shows results for biomedical natural language inference and semantic textual similarity tasks. Model with paraphrases for rare biomedical words can outperform the baseline in most cases. Paraphrases bring about up to 5\% improvement on average for few-shot learning with 16 training samples as to MedNLI task and 0.5\% increment with 256 training samples. We can see that pre-trained models tend to learn more about rare words with more training samples but paraphrases still act well. As to MedSTS, appended paraphrases are also shown as an effective strategy for most cases. In addition, tuning with paraphrases also generally improves model stability and reduces the variance of model prediction in few-shot scenarios.



==> _ACL Template-2/Text/5.Discussion.tex <==
\section{Discussion}

%\paragraph{Look up more rare words} In the above experiments, we only expand medical rare words in medical domain with meanings in the dictionary. For comparison, we also conduct experiments with paraphrases of rare words without domain restriction. However, the performance fluctuates around the baseline and fails to demonstrate coherence across different random seeds, which suggests looking up more r are word other than medical vocabularies in medical tasks isn't a better strategy.

% additional paragraph for camera-ready version
%\paragraph{Paraphrasing strategies} In Table \ref{number_of_rare_word} we can see that only a few paraphrases have been added into the training and development sets, especially with only 16 training samples. Therefore, we conduct the experiment with paraphrases for only test sets to explore the paraphrases in the training sets. Table \ref{table-only-test} shows that 
%\input{Table/only-test}




\paragraph{Train with more samples.} 
Apart from applying paraphrases in few-shot scenarios, we also attempt with more training samples for the MedNLI task, even with full-size training dataset. We attempt to sample the same number of development samples from the official MedNLI development set (with 1,395 samples) to match the number of training samples. If the training set is larger than the full-size development set, we just use the whole development set.
%Since we keep the training and development sets at the same size but there are only 1,395 samples in development set of MedNLI, we just utilize the full-size development set if the number of training samples is greater than 1,024. 

Table~\ref{mednli-more} demonstrates that our method outperforms the baseline on four out of six cases and performs comparably on the remaining two cases. When the whole training set is used, our model with paraphrases achieves 0.8\% improvement.
%with larger amount of training samples, our method can perform comparably with the baseline pre-trained models and the paraphrases can even achieve 0.8\% improvement with the full-size training set. 
The minor improvement might be attributed to the ``not so rare'' biomedical words as the rarity of words decreases during the expansion of training set, which helps the pre-trained models learn the semantics of the rare biomedical words better even without paraphrases.

\input{Table/more-data-mednli}

\paragraph{Which to look up?} 
Paraphrases can be helpful in general. However, for individual samples, that is not always the case. In Table~\ref{case-study}, we further scrutinize the cases where the model yields different predictions after adding the paraphrases. It is observed that the paraphrases can be less effective if the paraphrases of rare words are not task-related and critical for sentence understanding. For instance, in the third case in Table~\ref{case-study}, ``\textit{CHF}'' is a rare biomedical word which means ``\textit{congestive heart failure}''. Pre-trained models can easily match the hypothesis of ``\textit{poorly functioning}'' with the given premise. Otherwise, paraphrases can possibly introduce confusion. For example, in the wrong case in Table~\ref{case-study}, although ``\textit{workup}'' is a rare biomedical word in the pre-training corpora, it does not severely affect the semantics of the sentence and the pre-trained model turns to make wrong prediction with the misdirection from supplementary paraphrase.  %Experimental results show that paraphrases of rare words help training of pre-trained models even with fewer samples 

Actually, humans tend to continue reading unless the unknown words hinder the understanding. With this motivation, we believe that it is worthwhile to explore how to attach \textit{informative} paraphrases for the rare words, which will be investigated in future.

\input{Table/case-study}

%We display several cases in which model predicts differently with or without paraphrases of rare biomedical words from MedNLI in Table~\ref{case-study}. From the cases, we can see that paraphrases of rare biomedical words that are determinant in sentence understanding can be helpful to pre-trained model while paraphrases of those irrelevant rare biomedical words may confuse the model.



==> _ACL Template-2/Text/6.Conclusion.tex <==
\section{Conclusion}
Rare biomedical words are pervasive in biomedical texts, and understanding domain-specific rare words remains a tough challenge for pre-trained models.  In this work, we presented a simple yet effective method to help the pre-trained models grasp the semantics of rare biomedical words.

Enlightened by human reading behavior, we taught the pre-trained models to understand rare biomedical words by incorporating paraphrases of rare biomedical words. Our method can be regarded as a generic plug-in approach for prompt-based tuning without additional parameters. Experiments showed that our method could substantially improve the pre-trained models under few-shot settings.% and bring about plausible enhancement with more training data, even full-size of training set. 





==> _ACL Template-2/Text/7.Acknowledgement.tex <==
\section*{Acknowledgements}
% We thank the anonymous reviewers for their helpful and constructive comments and gratefully acknowledge the support of the National Key R\&D Program of China (2021ZD0113302) in the Technological Innovation ``2030 Megaproject''-New Generation Artificial Intelligence of China (2021ZD0113300) and the National Natural Science Foundation of China Youth Fund (62206079).

We thank the anonymous reviewers for their helpful and constructive comments and gratefully acknowledge the support of the National Key R\&D Program of China (2021ZD0113302) and the National Natural Science Foundation of China Youth Fund (62206079).

==> _ACL Template-2/Text/expi_Introduction.tex <==
\section{Introduction}
With the blossom of pre-trained models (PTMs), natural language processing (NLP) have been ushered into a new era \citep{peters2018deep,devlin2019bert,liu2019roberta,qiu2020pre}, along with that in biomedical domain tasks \citep{lee2020biobert,lewis2020pretrained,zhao2021recent}. However, there are two possible obstacles that may hinder the performance of biomedical PTMs, that are limited data and rare biomedical words.

In biomedical domain, it is common that the amount of data is limited due to rare diseases or data sensitivity \citep{vsuster2017short}. For instance, there are around 800 ICD codes in MIMIC-III dataset that have less than 40 hospital admissions while tha dataset contains 53,423 admissions overall \citep{johnson2016mimic}. Meanwhile, biomedical records are usually private data under confidentiality and biomedical data are not easily accessible. Promising results gained by ``Pre-training and Fine-tuning'' model are on the basis of sufficient training steps of additional parameters pertaining to new tasks, such as BERT \citep{devlin2019bert}. Otherwise, PTMs are unlikely to perform well in few-shot settings \citep{moradi2021gpt}. 

With limited tuning data for a new task, it is hard to fine-tune the PTMs and the new task-specific parameters effectively. To solve the above problem, ``Pre-training, Prompt and Predicting'' is proposed to smooth the fine-tuning process in few-shot settings by closing the gap between pre-training stage and the downstream task \citep{liu2021pre}. As demonstrated in Figure \ref{intro_prompt}, tuning with prompt inherits task paradigm from pre-training. Thus, downstream tasks wouldn't be a far cry from the pre-training tasks, which empowers the PTMs to perform better in the case of restricted amount of data.
% transfer to biomedical domain

Furthermore, quantity of specialized rare terms derive from Latin or Greek which are hard to comprehend \citep{keselman2012classification} for both human and PTMs. Besides, an increasing number of biomedical neologisms emerge over time due to biomedical breakthroughs or new diseases, like Covid-19. 

Also, words are generally in long-tail distribution and \citet{schick2020rare,wu2020taking} have discussed that rare words hinder the PTMs to understand sentences correctly. Biomedical rare words, which are semantically more related to biomedical tasks, tend to barrier the biomedical PTMs more. As an example of biomedical NLI task, model goes wrong when faced with a rare words ``\textit{afebrile}''\footnote{There are around 4 billion words in pre-training texts of the BC-RoBERTa-Large and ``afebrile'' appears only about 100,000 times. For comparison, the frequency of ``fever'' is 5 times that of ``afebrile''.} in the premise in Figure \ref{wrong-case} in Appendix \ref{appendix-wrong-case}, whose meaning is ``having no fever''. It's hard for PTMs to predict the label right without knowing ``afebrile''.

Several works alleviate the rare words problem in PTMs via leveraging non-rare words or tokens to approximate rare words \citep{schick2020rare} or injecting knowledge or contexts of certain set of rare words into pre-training procedure to enrich the representation of rare words \citep{yu2021dict,wu2020taking}. Although they have achieved improvement in grasping the meaning of rare words, further pre-training steps are essential for specific rare words. And if a trained model comes across new rare words in another task, extra pre-training will be inevitable. 
 

 


%More recently, PTMs are faced with a profound transformation from ``Pre-training and Fine-tuning'' to ``Pre-training, Prompt and Predicting'', namely prompt-based fine-tuning \citep{liu2021pre}. 

%Fine-tuning solves the downstream tasks with a transfer learning objective engineering from pre-trained targets, which requires sufficient training steps of additional parameters pertaining to new tasks, such as BERT \citep{devlin2019bert}. Although the model above is satisfactory to scenarios with adequate fine-tuning data, PTMs could not perform well in few-shot settings \citep{moradi2021gpt}. 

%Given this, tuning with prompt is proposed to transform downstream tasks from existing fine-tuning to look more like the pre-trained tasks by the help of \textit{prompt} \citep{liu2021pre}   
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{acl-ijcnlp2021-templates/Figure/intro-prompt-neo.pdf}
\caption{Examples for paradigms of (a) MLM (Masked Language Model) Pre-training. (b) Task-specific fine-tuning. (c) Prompt-based fine-tuning, with same task as pre-training process. (d) Paraphrase-enhanced prompt-based fine-tuning. Best viewed in color.}
\label{intro_prompt}
\end{figure*}




In this work, we build upon the recent success of prompt for the PTMs and focus on helping biomedical PTMs understand biomedical terms in the downstream tasks during tuning with prompt by looking them up in the dictionary, which mimics the behavior when human reads as knowledge enhancement. We attach the paraphrases of selected biomedical rare words to the words themselves in the datasets of downstream tasks only during tuning stage via tuning with vanilla prompt without 
extra pre-training. Also, our method is a plug-in module for task datasets and model-agnostic, which can be easily transferred to other domains and models\footnote{We plan to release our code at ...}.

In summary, our main contributions are as follows:
\begin{itemize}
    \item We are the first work to leverage paraphrases of words in the PTM tuning stage to enrich the representation, to the best of our knowledge.
    \item We combine the prompt-based fine-tuning and a portable plug-in module to help understand biomedical  rare words. Afterwards, we evaluate on two biomedical natural language understanding datasets and our approach can improve the performance by up to 5 \% in few-shot settings and 0.6 \% with full-size training dataset.
    \item We discuss how the paraphrases help with the PTMs and provide a novel perspective about task-related rare words.
    
\end{itemize}

==> _ACL Template-2/Text/x.ethics.tex <==
\section*{Ethical Considerations}
In this work, we propose an approach to explaining rare biomedical words for biomedical PTMs to help understand sentences with rare biomedical words. We conduct our experiments on the public biomedical datasets MedNLI and MedSTS with the authorization from the respective maintainers of the datasets. All experimental datasets involved have been de-identified by dataset providers and  only used for research.
